Word-order biases in deep-agent emergent communication

Sequence-processing neural networks led to remarkable progress on many NLP tasks. As a consequence, there has been increasing interest in understanding to what extent they process language as humans do. We aim here to uncover which biases such models display with respect to "natural" word-order constraints. We train models to communicate about paths in a simple gridworld, using miniature languages that reflect or violate various natural language trends, such as the tendency to avoid redundancy or to minimize long-distance dependencies. We study how the controlled characteristics of our miniature languages affect individual learning and their stability across multiple network generations. The results draw a mixed picture. On the one hand, neural networks show a strong tendency to avoid long-distance dependencies. On the other hand, there is no clear preference for the efficient, non-redundant encoding of information that is widely attested in natural language. We thus suggest inoculating a notion of "effort" into neural networks, as a possible way to make their linguistic behavior more human-like.

==> iconicity.tex <==
\subsection{Iconicity}
We contrast \emph{forward-} and \emph{backward-iconic} languages,
where phrases describe trajectory segments in the same/reverse order,
with non-iconic languages where the relation between segment and
phrase order is fixed by arbitrary (we randomly select 3 such
languages). Human language overwhelmingly prefer forward-iconicity,
so, if Seq2Seqs show similar constraints, they should show a preference
for this order both in terms of learning speed \cite[as is the case
for children][]{DERUITER2018202} and diachronic persistence. We
predict that backward-iconic, maintaining the same sequentiality as in
the trajectories, albeit in reverse order, should be easier than the
non-iconic languages. As markers are redundant with respect to fixed
word order, we expect, under standard least-effort assumptions
\cite{Zipf:1949}, that when testing agents as speakers they should
show a learning and preservation preference for no-markers languages,
whereas listeners might prefer the more robust cues in markers
languages.
% The second
% contrast that we look at is \textbf{Iconicity} vs
% \textbf{Non-Iconicity}. We build $2$ iconic languages;
% \textit{forward}-iconic and \textit{reverse}-iconic and $3$ non-iconic
% languages taken at random. We analyze then the contrast acquiring
% these languages with different architectures both in individual
% learning and iterated learning setup.  We anticipate a fast learning
% and long persistence through generations for the iconic languages as
% the agent can process the inputs sequentially. In contrast, non-iconic
% languages need more capacity by looking at non-ordered positions while
% processing. Aside from the processing argument, we see this contrast
% in children's perception at 5 years-old \cite{DERUITER2018202}. In our
% analysis, we look at the production and perception preferences of our
% agents.

\paragraph{Individual learning.} Fig.~\ref{fig:stats_FWO} shows test
accuracy during learning across. For the no-attention model, we observe a
clear preference for backward-iconic in both speaking and listening
mode. This is in line with the observation that Seq2Seq models in
machine translation work better when the source is presented in
reverse order \cite{Sutskever:etal:2014}. The (forward) iconic order
is better than the non-iconic ones in speaking only. Markers turn out
to help learning in both speaking and listening mode but, in line with
our prediction, they are more helpful when listening than
speaking. The attention-enhanced model shows much faster convergence
to perfect communication, that reaches perfect or near-perfect
accuracy within the first 20 epochs, which would not leave much room
for natural constraints to have an impact on learning: essentially, an
agent with attention can learn any language, irrespective of how
natural it is. Still we discern some sensible patterns in the initial
phases of learning. In speaking mode, the agent learns fastest with
the iconic language, followed by the backward-iconic one. The
non-iconic language without markers is the most difficult to learn, as
expected. Surprisingly, among the languages with markers, the
non-iconic one is actually easier than the iconic ones. Similar
patterns are observed for listener testing, but, in line with our
predictions, we don't observe a bias against languages with markers in
this setting.

% Similar to the previous result, attention and tying are speeding the learning substantially. Moreover, we have the same phenomenon regarding the ?? of architectures endowed with attention. The latter thus prevents the model from having meaningful biases. However, less powerful models with no attention prefer specific order, namely the reverse-iconic order followed by the iconic and finally the non-iconic order. This preference is present in the perception task which is aligned with children's preferences but also in the production task. Finally, the presence/absence of markers does not change this preference order.

\paragraph{Iterated Learning.} \textbf{Where are these results?} We
launch different generations each with a different source language and
we look at which language would degrade first. The result is
consistent with the model trends while learning as the easiest
language to learn, namely the reverse iconic language, is the most
resistant language requiring ?? generations before shifting followed
by the forward iconic language and then the non-iconic languages. This
confirms the preference for the iconic characteristic. \todo{...}


==> supplementary_controlLanguage.tex <==
\section{Controls for long-distance and local languages}

\todo{Specify the proportion of long/local, and explain what it is precisely that you are sampling? It is a set of phrase orders, that will be constant across all possible trajectories, right? Also, give examples. Discuss Table~\ref{supp:table:examples_local} and \ref{supp:table:examples_long}}

As the long-distance language includes all utterances from the local language, it might be trivially harder to learn. To account for this, we construct $3$ control languages by randomly sampling, for each trajectory, the same number of possible utterances for the local and long-distance controls. In other words, for long-distance controls, we sample $m$ constructions,  by keeping the same proportion of local and long-distance constructions in the original long-distance language, to match the number of possible sampled utterances in the local-distance controls. Note that this number $m$ depends on the number of segments. Practically, we sample randomly $24$ possible combinations for $3$ length segments (all with local utterances for local-distance control languages and $16$ with long-distance and $8$ with local utterances for long-distance control languages) , $4$ combinations for 2-length segments and $2$ combinations for 1-length segments. 

%\begin{itemize}
%\item long distance
%  \begin{itemize}
%  \item 3-segment instructions: $144$ combinations: with $96$ combinations with $2$ length-dependency (LD) and $48$ with $0$LD
%  \item 2-segment instructions: $16$ combinations: $8$ combinations with $2$LD and $8$ with $0$LD
%  \item 1-segment instructions: $2$ combinations: $0$ combinations with $2$LD and $2$ with $0$LD
%  \end{itemize}
%\item local distance
%  \begin{itemize}
%  \item 3-segment instructions: $48$ combinations all with $0$LD
%  \item 2-segment instructions: $8$ combinations all with $0$LD
%  \item 1-segment instructions: $2$ combinations all with $0$LD
%  \end{itemize}
% \end{itemize} 
%Based on those languages we create control languages with have the same number of combinations for the long and local structures:
%\begin{itemize}
%\item long distance control
%  \begin{itemize}
 %   \item 3-segment instructions: $24$ combinations taken at random without replacement from $144$: $16$ combinations with $2$LD and $8$ with $0$LD. Note that we keep the same proportion of $0$ and $2$ LD of the original language.
%  \item 2-segment instructions: $4$ combinations: $2$ combinations with $2$LD and $2$ with $0$LD
%  \item 1-segment instructions: $2$ combinations: $0$ combinations with $2$LD and $2$ with $0$LD
%  \end{itemize}
%\item local distance control
%  \begin{itemize}
%  \item 3-segment instructions: $24$ combinations all with $0$LD
%  \item 2-segment instructions:$4$ combinations all with $0$LD
%  \item 1-segment instructions: $2$ combinations all with $0$LD
  %\end{itemize}
%\end{itemize}

%We construct $3$ different controls for each structure by sampling from the original language to make sure that our results do not depend on the chosen combinations.


==> supplementary_earlyStopping.tex <==
\subsection{The effect of early stopping in the distribution for Free order languages}
Starting iterative learning with a free word order (with markers) showed a shift from the uniform ground truth distribution to a more skewed one. We even observe this phenomenon from generation $0$. This is due to the early stopping that we impose during training. Figure \ref{fig:earlyStopping} shows the same model trained individually with early stopping (left) and to $100$ epochs (right). Both of those models have $100\%$ accuracy but the first model has a more peaked distribution with an entropy of $4.76$ compared to the second model with an entropy of $4.78$. Thus, we observe the shift from the ground truth distribution caused by the miss-match between the loss function pushing the model to fit the ground-truth distribution and the stopping criteria during evaluation that assesses the communication success. This shift becomes stronger through generations as the distribution to fit becomes less uniform.
\begin{figure}
\centering
    \includegraphics[width=\columnwidth]{figs/earlyStopping.eps}
    \caption{Distribution after convergence of models trained individually. The solid dots depict all possible order combinations that can be used to describe five-segment trajectories, sorted by their frequency (seen as a line). The dotted red line corresponds to the uniform distribution over all combinations. The most (least) frequent combination and its closest neighbours are represented by green dots (red squares).}\label{fig:earlyStopping}
\end{figure}


==> supplementary_iconicityRank.tex <==
\subsection{Diachronic persistence of iconic orders}

The iterative learning experiment seeded with free word-order (with markers) showed a shift from the uniform distribution of word orders.  We examine in this part some characteristics of this shift, in particular, whether backward and (forward) iconic utterances are favored through generations. We expect, that as those orders are easy for agents to acquire (fast convergence during the individual learning), they should be pushed to lower ranks through the process of evolution \footnote{Lower rank means more likely to be produced}. Practically, we launch $15$ different iteration processes starting from $3$ different seeded parents (each parent has $5$ direct children, which on their turn would have only one direct child each). Figure \ref{fig:ranks} shows the rank of production the iconic utterances. Surprisingly, we observe that the (forward) iconic order is pushed to higher ranks over generations for most seeds.  For the backward order however, we don't observe a clear pattern. The latter seems to have less variant ranks through generations, but still in contrast with our expectation, it not pushed for lower ranks. 

\begin{figure}[ht]
\centering
    \includegraphics[width=\columnwidth]{figs/ranks.eps}    

\caption{Rank of the production of forward (up) and backward (down) iconic orders through generations across different seeds. Each segment represents an agent and its direct successor and each color represents one iterative process from generation $0$ to $7$.}\label{fig:ranks}
\end{figure}


==> word_order.tex <==
\subsection{Fixed word order vs.\ markers}
We next consider whether we encounter the expected trade-off between
expressing the relation between phrases with fixed word order or
through markers. A free-word-order language without markers should be
impossible to learn. More interestingly, free word order with marker
and fixed word order without markers should be easier to learn and more stable
in diachrony than languages redundantly coding roles with word order
\emph{and} markers. Finally, the complete, equiprobable phrase order
freedom of our languages is unlike what is encountered even in
non-configurational languages, where certain orders are always at
least statistically favored \cite{Hale:1992,Mithun:1992}. We thus
predict that, across generations, free word order will become more
fixed, with some preferred orders emerging.

% We train the agents with simple languages that possess a contrast between \textbf{Fixed-Order} vs \textbf{Free-Order}. Specifically, we consider languages with Free-Order with markers (\textbf{Free+M}) and without markers (\textbf{Free-M}) and compare them with multiple Fixed-Order languages also with markers (\textbf{Fix+M}) and without markers (\textbf{Fix-M}). We expect the agents to perform at the chance level on  \textbf{Free-M} as this language is ambiguous. Indeed, a fixed word order and case marking can ease the processing of sentence semantics and reduce ambiguity and should then be easier than \textbf{Free-M}. Moreover, to draw the parallel with natural language, some languages evolved from \textbf{Free+M} to \textbf{Fix-M}. To give a concrete example, we can look at French and its ancestor, Latin. In Latin, the endings of nouns, verbs, adjectives, and pronouns allow for extremely flexible order in most situations. In contrast, French has a strict word order. French , thus, evolved from Latin and lost the flexibility of word order through the lost of case marking. In this section we will look at whether those contrasts that we see in Humans are present in LSTMs. We will first examine this in individual learning setup, then in an iterated learning setup starting with the \textbf{Free+M} (simulating Latin) and look at the properties of the child language.

\paragraph{Individual learning.} We first confirmed that the
free-order language without markers could not be learned by either
model (performance still at chance level after 100 epochs). The
variant with markers is reported in Fig.~\ref{fig:stats_FWO}. The
no-attention agent can learn to parse this language reasonably well
within a span of 100 epochs (listening mode), but a much longer
learning time is needed to learn to produce it \textbf{(how many
  epochs?)}.  When listening, the agent is presented with an utterance
in arbitrary order to be deterministically translated into a
trajectory. When speaking, it is the job of the agent to pick one of
the possible orders. This is evidently a more challenging task
(despite the fact that, in the evaluation, \emph{any} acceptable order
would be positively scored). We are not aware of production-perception
asymmetries in human learning of non-configurational languages, but
this might be an interesting avenue of future research. The prediction
of a trade-off that should lead to prefer free order with markers or
fixed without is not borne out, as there is a general preference for
the redundant languages over the alternatives, in both
directions. Attention again makes learning of the free-order language
possible in both directions, and even fast. Again, we don't observe a
tendency to prefer non-redundant coding.

 % Agents are trained to speak and listen in a particular language with a specific property that we want to look at (\textbf{Free+M}, \textbf{Free-M}, \textbf{Fix+M} and \textbf{Fix-M}). Figure \ref{fig:stats_FWO} shows the accuracy during the learning process on the validation dataset for different architectures. First, attention is speeding learning substantially. Moreover, as expected, tying the input and output layers pushes the agent to acquire faster the different languages. We think that this is because training the \emph{Listener} and the \emph{Speaker} are helping each other. But what is interesting is that even if agents with no attention are slower, they have meaningful biases toward some properties. In fact, \emph{Speakers} without attention have a clear preference for \textbf{fixed-order} compared to \textbf{Free+M}. However, for the perception part, this property doesn't seem very important. Also for those type of models, tying changes the preference for some properties. In fact, \textbf{Markers} are always helpful for the listening part. But this is not always the case for production. Indeed, when embeddings are tied, \emph{Speakers} and \emph{Listeners} have the same preferences, and if they are not, \emph{Speakers} are faster producing languages with no \textbf{Markers}. Finally, agents endowed with attention do not have any of those contrasts as they handle all the languages with equal ease. Which leads us to conclude that attention is a powerful mechanism that disfavors the emergence of meaningful biases.

\paragraph{Iterated learning.}  \textbf{Points to be discussed here: is free word order with markers less stable than iterated learning, with and without attention, and in speaking and listening? are fixed languages with markers less stable than either fixed languages without markers and free word order? for free word order, what happens across generations? does it converge to a few languages? what are they? do markers get lost in the way? } We concluded in the previous paragraph that some architectures have meaningful inductive bias preferring \textbf{fixed-order} languages to \textbf{free-order}. We choose one of those architectures to simulate the evolution of the \textbf{Free+M} language. More specifically, we take agents with tied embeddings and no attention as they demonstrate meaningful bias \textbf{(no longer convinced of this claim, do the results change with attention?)} and learn fast different languages. We seed different agents with \textbf{Free+M} and pair them, as parents, with new child-agents, also with the same architecture. We continue this process, called iterated learning, for multiple generations.  Figure \ref{fig:FWO_iterated} shows the distribution over the possible combinations produced by agents on $5$ segments trajectories ($120$ possible combinations) after convergence at different stages of the iterated learning process. We examine first the distribution of generation $0$. Agents of generation $0$ are trained to fit the uniform distribution. Formally, for each input $\vt$, \emph{Speakers} need to output $\vu \sim U_{\textbf{fixed+M}}$. This distribution corresponds to the dashed line in the figure \ref{fig:FWO_iterated}. We notice that generation $0$, even if it has a perfect accuracy, does not simulate perfectly the dataset. First, it has a slight preference outputting some orders compared to others. Second, this preference is not completely arbitrary. In fact, if we look at the most likely combination, we notice that its neighbors are also likely (green dots). In the same manner, the least likely combination's neighbors are also unlikely (red squares). That means that the model is optimizing for a trade-off between its objective function and its biases. Of course, training the agent for a longer time would lead to a complete drift from its biases and a perfect fit of the distribution. \dpx{This is not proven, right? It could never converge...} \textbf{Should we talk about poverty of stimulus and Chomsky theory here to justify why we don't train the models forever? Maybe also say that this is obtained with early stopping on the dev set so it is actually perfect}. \dpx{I dont understand the relevance of poverty of the stimulus in this context; of course, we cannot run a computer forever, and hence a stopping rule is necessary; the one you've defined is perfectly ok.} Then when we go deeper in the generations, we notice that the distribution becomes more skewed as the entropy decreases. In other words, the child language is drifting toward more fixed-order language over generations. Finally this drift goes along with maintaining, even emphasizing, the neighbors' clusters.
\todo{say we have the same results with attention too}. \todo{add entropies for fig 3: entropy of $4.783$, $4.775$, $4.744$, $4.694$ and $4.670$.}

\begin{figure}
\centering
    \includegraphics[width=\columnwidth]{figs/FWO_iterated_acc_seed2.eps}
    \caption{The evolution of combinations' frequency in the agents' outputs. The solid dots depict all possible order combinations that can be used to describe five-segment trajectories, sorted by their frequency (seen as a line). The dotted red line corresponds to the uniform distribution over all combinations. The most (least) frequent combination and its closest neighbours are represented by green dots (red squares).}\label{fig:FWO_iterated}
\end{figure}

